Formalising opencypher Graph Queries in Relational Algebra

Graph database systems are increasingly adapted for storing and processing heterogeneous network-like datasets. However, due to the novelty of such systems, no standard data model or query language has yet emerged. Consequently, migrating datasets or applications even between related technologies often requires a large amount of manual work or ad-hoc solutions, thus subjecting the users to the possibility of vendor lock-in. To avoid this threat, vendors are working on supporting existing standard languages (e.g. SQL) or creating standardised languages. In this paper, we present a formal specification for openCypher, a high-level declarative graph query language with an ongoing standardisation effort. We introduce relational graph algebra, which extends relational operators by adapting graph-specific operators and define a mapping from core openCypher constructs to this algebra. We propose an algorithm that allows systematic compilation of openCypher queries.

==> alg-build-rga-tree.tex <==
% FIXME: if used, correct wording: query part -> single query, subquery -> query part
\begin{algorithm}[htb]
  \DontPrintSemicolon
  \KwData{$P$ is the list of query parts}
  $R \leftarrow []$ \tcp*[r]{empty list to hold compiled form of query parts}
  \ForEach{query part $p \in P$}{
    $t \leftarrow \textit{None}$ \tcp*[r]{\rga tree built so far}
    \ForEach{subquery $s \in p$}{
      $t \leftarrow \KwFnBRSQ(s, t)$
    }
    $R \leftarrow R + [t]$
  }
%  \eIf(\tcp*[f]{only one query part: no need to union}){$|R| = 1$}{
%    \Return $R[0]$ \;
%  }{
%    \Return $\unionop(R)$ \;
%%	\item Process each query part as follows and combine their result using the \uniontext opertaion. As the \uniontext operator is technically a binary operator, the \uniontext of more than two query parts are represented as a left deep tree of \lstinline+UNION+ operators.
%  }
  \Return $\unionop(R)$ \;
  \caption{Build relational graph algebra tree from openCypher query.}
  \label{alg:build-rga-tree}
\end{algorithm}


==> alg-build-subquery-tree.tex <==
% FIXME: if used, correct wording: subquery -> query part
\begin{algorithm}[htb]
  \DontPrintSemicolon
  \KwData{$s$ is the subquery to compile}
  \KwData{$\mathit{tree}$ is the \rga of the subqueries so far}
  \Fn{\KwFnBRSQ{s, tree}}{
    Combine using $\joinop$: \Begin{
      \ForEach{\lstmatch\ clause $m \in s$}{
        Combine using $\joinop$ or $\leftouterjoinop$: \Begin(\tcp*[f]{$\leftouterjoinop$ for \lstinline+OPTIONAL MATCH+}){
          \ForEach(\tcp*[f]{comma separated patterns}){ $pat \in m$}{
            Turn $pat$ left-to-right to a \getverticestext for the first vertex and a chain of \expandintext, \expandouttext or \expandbothtext operators for inbound, outbound or undirected relationships, respectively.
          }
	  }
        $\alldifferentop(.)$ \tcp*[r]{edge variables in patterns of $m$}
	  \If{$m$ has \lstwhere\ subclause}{
	    $\selectionop(.)$ deferring positive or negative patterns as $d$ \;
        }
      }
    }
    \lIf{positive pattern deferred}{$(.)\joinop(d)$}
    \lIf{negative pattern deferred}{$(.)\antijoinop(d) $}
    \lIf{tree is not None}{ $t \joinop(.)$ }
    \eIf{\lstreturnwith has grouping function}{
      $\gc \leftarrow \KwFnDGC(\mathit{items}\ \mathit{in}\ \lstreturn)$ \;
      $\groupingop_\gc(.)$ \;
    }{
      $\projectionop(.)$
    }
    \lIf{\lstreturnwith has \lstdistinct}{ $\duplicateeliminationop(.)$ }
    \lIf{\lstreturnwith has \lstwhere}{ $\selectionop(.)$ }
    \Return $.$
  }
  \caption{Build \rga from subquery.}
  \label{alg:build-subquery-tree}
\end{algorithm}


==> evaluation.tex <==
\section{Evaluation}

Akka toolkit~\cite{Akka}, which uses the actor concurrency model~\cite{butcher2014seven}


==> preliminaries.tex <==
% !TeX spellcheck = en_GB
% !TeX encoding = UTF-8
\section{Preliminaries}
\label{sec:preliminaries}

This section defines the mathematical concepts used in the paper. Our notation closely follows~\cite{DBLP:conf/edbt/HolschG16} and is similar to~\cite{DBLP:books/igi/Sakr11/RodriguezN11}. %\footnote{The formalism presented in~\cite{DBLP:books/igi/Sakr11/RodriguezN11} lacks the notion of \emph{vertex labels}.}.


\paragraph{Summary.} \autoref{table:operators} provides an overview of the operators of \rga.



==> property-graph-example.tex <==
\footnotesize
\begin{minipage}{0.55\linewidth}
$V = \{a, b, c, d, e, f\}; E=\{1, 2, 3, 4, 5, 6, 7\}$

$\verticestoedges(1) = \tuple{a, b}; \verticestoedges(2) = \tuple{b, c}; \ldots$

$\vertexlabels = \{\atom{Person}, \atom{Message}, \atom{Post}, \atom{Comment}\};$

$\edgelabels = \{\atom{KNOWS}, \atom{LIKES}, \atom{REPLY\_OF}\}$

$\vertexlabelfunction(a) = \{\atom{Person}\}; \vertexlabelfunction(d) = \{\atom{Message}, \atom{Post}\}; \ldots$

$\edgelabelfunction(1) = \atom{KNOWS}; \edgelabelfunction(3) = \atom{LIKES}; \ldots$

$\vertexproperties = \{\atom{name}, \atom{speaks}, \atom{language}\};$

$\edgeproperties = \{\};$

$\propertyfunction{name}{a} = \atom{'Alice'}; \propertyfunction{name}{b} = \atom{'Bob'}; \ldots$

$\propertyfunction{title}{1} = \relnull; \propertyfunction{title}{2} = \atom{}; \ldots$

$\propertyfunction{release}{1} = \relnull; \propertyfunction{release}{2} = \atom{}; \ldots$
\end{minipage}


==> relalg-multiple-subqueries.tex <==
\begin{forest} for tree={align=center}
	[
	{$\projection{\var{m2.language}\assign \var{reply},~\var{m3.language}\assign \var{orig}
		}{}
		$
	}
	[
	{$\leftouterjoin$
	}
	[
	{$\selection{
			\var{m2.language} = \var{singleLang}
		}
		$
	}
	[
	{$\join$
	}
	[
	{$\selection{
			\var{cnt} = \literal{1}
		}
		$
	}
	[
	{$\grouping{\var{m1.language}\assign \var{singleLang}, \literal{count(*)}
			\assign \var{cnt}}{\var{m1.language}}$
	}
	[
	{$\getvertices{m1}{Message}$
	},tier=input,for tree={blue,densely dashed}
	]
	]
	]
	[
	{$\getvertices{m2}{Message}$
	},tier=input,for tree={blue,densely dashed}
	]
	]
	]
	[
	{$\expandout{m2}{m3}{Message}{\_e1}{REPLY\_OF}{1}{1}$
	}
	[
	{$\getvertices{m2}{Message}$
	},tier=input,for tree={blue,densely dashed}
	]
	]
	]
	]
	;
\end{forest}


==> relalg-selection1.tex <==
$$
\projection{\var{p1.name}, \var{p2.name}
}{}
\selection{
	\var{k.since} < \literal{2000}
}
\expandboth{p1}{p2}{Person}{k}{KNOWS}{1}{1}
\getvertices{p1}{Person}
$$


==> relalg-selection2.tex <==
$$\projection{\var{p.speaks}
}{}
\selection{
	\var{p.name} = \literal{"Bob"}
}
\getvertices{p}{Person}
$$


==> relalg-triangle.tex <==
\begin{align*}
\begin{autobreak}
\projection{\var{p1}, \var{p2}, \var{m}
}{}
\Big(
\alldifferent{\var{\_e2}, \var{\_e3}, \var{\_e1}}\Big(
\expandout{p2}{m}{Message}{\_e3}{LIKES}{1}{1}\Big(
\expandboth{p1}{p2}{Person}{\_e2}{}{1}{1}\Big(
\expandin{m}{p1}{Person}{\_e1}{LIKES}{1}{1}\Big(
\getvertices{m}{Message}
\Big)
\Big)
\Big)
\Big)
\Big)
\end{autobreak}
\end{align*}
